M2Lingual: Enhancing Multilingual, Multi-Turn Instruction Alignment in Large Language Models

Instruction finetuning (IFT) is critical for aligning Large Language Models (LLMs) to follow instructions. While many effective IFT datasets have been introduced recently, they predominantly focus on high-resource languages like English. To better align LLMs across a broad spectrum of languages and tasks, we propose a fully synthetic, novel taxonomy (Evol) guided Multilingual, Multi-turn instruction finetuning dataset, called M2Lingual. It is constructed by first selecting a diverse set of seed examples and then utilizing the proposed Evol taxonomy to convert these seeds into complex and challenging multi-turn instructions. We demonstrate the effectiveness of M2Lingual by training LLMs of varying sizes and showcasing the enhanced performance across a diverse set of languages. We contribute the 2 step Evol taxonomy with the guided generation code: https://github.com/ServiceNow/M2Lingual, as well as the first fully synthetic, general and task-oriented, multi-turn, multilingual dataset built with Evol - M2Lingual: https://huggingface.co/datasets/ServiceNow-AI/ M2Lingual - containing 182K total IFT pairs, covering 70 languages and 17+ NLP tasks.

==> Tables/taxonomy-table.tex <==




% \begin{table}[ht]
% \centering
% \tiny
% \begin{tabular}{>{\raggedright\arraybackslash}p{3cm}>{\raggedright\arraybackslash}p{10cm}}
% \toprule
% \textbf{Task} & \textbf{Type of Evolves} \\
% \midrule
% Generic Prompts & Transliteration, Dialect, Concise, Deepen, Concretize, Increase Reasoning \\
% \midrule
% Abstractive Summarization Prompts & Adding Distractors, Technical Jargon, Inconsistencies In Information, Multiple Topics, Metaphors Idiom, Long Distance, Multiple Languages, Unstructured Data, Personal Opinion \\
% \midrule
% Reranking Tasks & Cross Lingual, Domain Language, Emotional Subtext, Need For Context, Ambiguity In Wording, Long Text, Idiom Slang, Adding Distractors, Multiple Questions \\
% \midrule
% Commonsense Physical Reasoning & Object Interaction, Object Properties, Logical Sequencing, Object Transformation, More Choices, Justification, Incorrect Choices, Double Negatives, Theoretical Scenario \\
% \midrule
% Opendomain Qa & Ambiguity, Long Form Question, Multilingual, Combine Facts, Implicit Question, Negative Questions, Inference Deduction, Multiple Answers, Comparitive Questions \\
% \midrule
% Cross Lingual Summary & Adding Distractors, Technical Jargon, Inconsistencies In Information, Multiple Topics, Metaphors Idiom, Long Distance, Cross Lingual Summary, Unstructured Data, Personal Opinion \\
% \midrule
% Pawsx & Idioms Phrases, Abbrevations, Sentence Structure, Information, Variation, Negation, Time Navigation, Cultural Inferences, Length Variation \\
% \midrule
% Flan Cot & Complex Jargon, Multiple Languages, Long Complex Queries, Disconnected Clues, Emotion Sarcasm, Advanced Reasoning, Ambiguity, Unknown Context, Implicit Bias \\
% \midrule
% Adversarial Qa & Complex Question, Advanced Vocab, Multiple Themes, Ambiguity, More Details, Increase Reasoning, Time, Abstract Topics, Structured Info \\
% \midrule
% Mintaka & Ambiguity, Long Form Question, Multilingual, Combine Facts, Implicit Question, Negative Questions, Inference, Multichoice Questions, More Reasoning \\
% \midrule
% Flan Qa & More Choices, More Complex, Negation, Multiple Correct Options, Need For Context, Justification, Distracting Long, Close Choices, No Correct Option \\
% \midrule
% Joke Explain & Jargon, Slang, Cultural References, Non Explicit Punchline, Time Bound, Compound Jokes, Language, Long, Double Entendre \\
% \midrule
% Soda Inst & Genre Specific, Character Constraints, Setting Restrictions, Plot Twists, Narrative Style, Word Count Limit, Incorporate Dialogue, Theme Integration, Include Symbolism \\
% \midrule
% Flan Coqa & Ambiguity, Long Form Question, Multilingual, Combine Facts, Implicit Question, Negative Questions, Inference, Multichoice Questions, More Reasoning \\
% \midrule
% Flan Lambda & Multiple Blanks, Contextual Blanks, Word Bank, Missing Letters, Grammar Forms, Logical Inferences, Word Classes, Synonyms Antonyms, Cultural Context \\
% % \midrule
% % Follow Up Scripts & Challenging Follow Up, Ambiguous Follow Up, Redirection Follow Up, Generic Rewriting Follow Up, Feedback Handling Follow Up, Random Follow Up, Context Retention Follow Up, Format Rewriting Follow Up, Persona Rewriting Follow Up, Detailed Constraints, Adjust Output Format, Expanding Queries, Refocus Queries, Change Context, Clarification, Chatbot Opinion, Open Ended Questions, Complex Queries, Pronouns, Engaging Conversation, Recall Information \\
% \bottomrule
% \end{tabular}
% % \vspace{0.2cm}
% \label{tab:taxonomy}
% \caption{Tasks and their evolves. For MLQA, HotpotQA and Dolly split in the Aya collection we use the prompts used for Mintaka, Opendomain QA and Generic instructions respectively.}
% \end{table}








% Mlqa & (Same as Mintaka) \\
% \hline
% Hotpotqa & (Same as Opendomain Qa) \\
% \hline
% Dolly & (Same as Generic Prompts) \\
% \hline
